ShabbyPages: A Reproducible Document Denoising and Binarization Dataset

Document denoising and binarization are fundamental problems in the document processing space, but current datasets are often too small and lack sufficient complexity to effectively train and benchmark modern data-driven machine learning models. To fill this gap, we introduce ShabbyPages, a new document image dataset designed for training and benchmarking document denoisers and binarizers. ShabbyPages contains over 6,000 clean "born digital" images with synthetically-noised counterparts ("shabby pages") that were augmented using the Augraphy document augmentation tool to appear as if they have been printed and faxed, photocopied, or otherwise altered through physical processes. In this paper, we discuss the creation process of ShabbyPages and demonstrate the utility of ShabbyPages by training convolutional denoisers which remove real noise features with a high degree of human-perceptible fidelity, establishing baseline performance for a new ShabbyPages benchmark.

==> oldbib.tex <==
\begin{thebibliography}{8}
\bibitem{ref_Kaggle}
  https://www.kaggle.com/datasets
\bibitem{ref_HuggingFaceHub}
  {https://huggingface.co/datasets}
\bibitem{ref_RDCL2019}
{Christian Clausner, RDCL2019 Competition Dataset (Recognition of Documents with Complex Layouts) (RDCL2019) ,1,ID:RDCL2019\_1,URL:https://tc11.cvc.uab.es/datasets/RDCL2019_1}

\bibitem{ref_Tobacco800}
{David Doermann, Tobacco 800 Dataset (Tobacco800) ,1,ID:Tobacco800_1,URL:https://tc11.cvc.uab.es/datasets/Tobacco800_1}

\bibitem{ref_icdar}
{Harold Mouchère, ICDAR 2019 Competition on Recognition of Handwritten Mathematical Expressions and Typeset Formula Detection (ICDAR2019-CROHME-TDF) ,1,ID:ICDAR2019-CROHME-TDF\_1,URL:https://tc11.cvc.uab.es/datasets/ICDAR2019-CROHME-TDF_1}

\bibitem{ref_NoisyOffice}
{Castro-Bleda, MJ.; España Boquera, S.; Pastor Pellicer, J.; Zamora Martínez, FJ. (2020). The NoisyOffice Database: A Corpus To Train Supervised Machine Learning Filters For Image Processing. The Computer Journal. 63(11):1658-1667. https://doi.org/10.1093/comjnl/bxz098}

\bibitem{ref_RVL-CDIP}
  @article{DBLP:journals/corr/HarleyUD15,
  author    = {Adam W. Harley and
               Alex Ufkes and
               Konstantinos G. Derpanis},
  title     = {Evaluation of Deep Convolutional Nets for Document Image Classification
               and Retrieval},
  journal   = {CoRR},
  volume    = {abs/1502.07058},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.07058},
  eprinttype = {arXiv},
  eprint    = {1502.07058},
  timestamp = {Mon, 13 Aug 2018 16:48:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/HarleyUD15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

\bibitem{ref_NoisyOfficeDatabase}
{F. Zamora-Martinez, S. España-Boquera and M. J. Castro-Bleda, Behaviour-based Clustering of Neural Networks applied to Document Enhancement, in: Computational and Ambient Intelligence, pages 144-151, Springer, 2007.}

\bibitem{ref_UCIMLR}
{Dua, D. and Graff, C. (2019). UCI Machine Learning Repository [http://archive.ics.uci.edu/ml]. Irvine, CA: University of California, School of Information and Computer Science.}

\bibitem{ref_DocCreator}
  {Journet Nicholas, Visani Muriel, Mansencal Boris, Van-Cuong Kieu, Billy Antoine, DocCreator: A New Software for Creating Synthetic Ground-Truthed Document Images. J. Imaging 2017, 3, 62.}
\bibitem{ref_goldmann}
  {Pau Riba, Anjan Dutta, Lutz Goldmann, Alicia Fornes, Oriol Ramos, Josep LLados: "Table Detection in Invoice Documents by Graph Neural Networks", ICDAR, 2019.}
\bibitem{ref_zenodo}
  {Layout Analysis Groundtruth for the RVL-CDIP Dataset. Goldmann, Lutz. 10.5281/zenodo.3257319}
\bibitem{ref_tobacco800gt1}
  {Guangyu Zhu, Yefeng Zheng, David Doermann,and Stefan Jaeger. Multi-scale Structural Saliency for Signature Detection. In Proc. IEEE Conf. Computer Vision and Pattern Recognition (CVPR 2007), pp. 1‐8, 2007.}
\bibitem{ref_tobacco800gt2}
  {Guangyu Zhu and David Doermann. Automatic Document Logo Detection. In Proc. 9th Int. Conf. Document Analysis and Recognition (ICDAR 2007), pp. 864‐868, 2007.}
